Synthesizing Anyone, Anywhere, in Any Pose

We address the task of in-the-wild human figure synthesis, where the primary goal is to synthesize a full body given any region in any image. In-the-wild human figure synthesis has long been a challenging and under-explored task, where current methods struggle to handle extreme poses, occluding objects, and complex backgrounds. Our main contribution is TriA-GAN, a keypoint-guided GAN that can synthesize Anyone, Anywhere, in Any given pose. Key to our method is projected GANs combined with a well-crafted training strategy, where our simple generator architecture can successfully handle the challenges of in-the-wild full-body synthesis. We show that TriA-GAN significantly improves over previous in-the-wild full-body synthesis methods, all while requiring less conditional information for synthesis (keypoints \vs DensePose). Finally, we show that the latent space of TriA-GAN is compatible with standard unconditional editing techniques, enabling text-guided editing of generated human figures.

==> tex/face_sticking.tex <==
\section{Face sticking artifacts}
The CSE-guided generator seems generate images that "sticks" to the CSE textures.
This was observed for the DeepPrivacy face generator as well, where eyes would "stick" to the keypoint.


\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{figures/face_sticking/face_consistency2.png}
    \includegraphics[width=.8\textwidth]{figures/face_sticking/face_consistency3.png}
    \includegraphics[width=.8\textwidth]{figures/face_sticking/face_consistency4.png}
    \includegraphics[width=.8\textwidth]{figures/face_sticking/face_consistency5.png}
    \caption{
        The generated images with CSE-textures seem to "stick" to the CSE textures.
    }
\end{figure}

==> tex/larger_model.tex <==


\section{Larger Models}

\paragraph{Progressive Training / Curriculum training}
Progressively training a generative model, by first training a low-resolution model (\eg 16x16, 32x32) then progressively increasing the resolution.
There exists several adaptions:

\begin{itemize}
    \item Progressive growing of GANs (PG-GAN) \cite{Karras2017}. Train at 16x16 resolution, then progressively increase resolution to 32x32 by linearly interpolating low-resolution with high resolution image.
    \item StyleGAN-XL \cite{Sauer22XL} freezes the low resolution model, removes a couple of layers of it and train a number of super-resolution stages.
    Note that these models depend on eachother, and can't be trained in parallel.
    \item Cascaded diffusion models (CDM) \cite{Ho2022} trains a base model that generates 32x32 image, then a  set of super-resolution models.
    The training of super-resolution stages is done via mapping the real data (bilinearly downsampled) to the higher-resolution image.
    Therefore, the training can be done independently and in parallel.
\end{itemize}


Progressive methods: progressively fill in the image \cite{Li_2020RFR} 

Two-stage inpainting approaches are widely adopted for image inpainting, where the typical case is to generate a low-resolution image then refine the low resolution image (\cite{Zeng2020}, \cite{Yu2018GConv}, \cite{Yu2018ContextualAttention}).
These methods optimize the L1 loss for the coarse networks.
Other work propose to first predict a semantic structure of the image, via "structure maps" \cite{Ren_2019}, edges \cite{Nazeri_2019b}, saliency maps \cite{Xiong2019}.


\hhnote{Check what the authors \cite{Ren_2019} call "Structure maps".
Not sure if "saliency maps" refers to foreground-background. Often saliency refers to where people/networks focus in an image.}


CDM \cite{Ho2022} simplifies training. However, it requires a large amount of parameters, and it is not applied to an image-to-image problem before.
For example, high-resolution details in the conditioning image might be  lost in downsampling, which could be crucial for the base model.
The benefit of CDM is removing the missing-value problem for higher resolutions.

\paragraph{Architecture ablations on U-net}

\begin{itemize}
    \item \cite{imagen2022}
    \item \cite{dhariwal2021}
\end{itemize}




\subsection{Gated U-Nets}
The U-net \cite{Ronneberger2015} architecture is widely adopted for image-to-image architectures, including GANs, diffusion models, and image inpainting models.
For image inpainting, the U-net architecture is often not adopted \cite{Suvorov22LAMA,Yu2018GConv}, and found nonessential \cite{Yu2018GConv}.
Probably, this is caused by transferring the missing value problem from the encoder to the decoder.
However, simply leaving out the u-net connection removes the benefit of its improved gradient flow to early layers of the encoder, and the direct transfer of high-level texture and structural information from the input.


We propose a gated U-net skip connection for higher resolution feature maps.
Given a feature map from the encoder, $y$, and from the decoder $x$, we define the U-net skip connection as,
\begin{equation}
    f(x, y) = x + (s(x,y) \cdot y + (1 - s(x,y)) \cdot x),
    \label{eq:gated_unet}
\end{equation}
where $s(x,y) = \sigma (\text{conv}(\text{cat}(x,y)))$, and $\sigma$ is the sigmoid activation function.
Note that $f$ acts as a residual connection, where the decoder feature map has a direct gradient path through $f$ to $x$ to prevent vanishing gradients.
We replace all u-net skip connections with \cref{eq:gated_unet} for feature map resolutions larger than $16 \times 16$.
\cref{eq:gated_unet} is a straightforward connection that learns to propegate known pixels to the decoder layers.
There are numerous task-specific skip connections for image inpainting \cite{Yi_2020,Yan2018ShiftNet,Liu2020,Zeng2022AOT,Hukkelas21IP,Zeng2022AOT}.
In contrast to previous methods, \cref{eq:gated_unet} is a residual connection preventing vanishing gradients and is straightforward to implement.

\hhnote{Add pseudocode?}
\begin{itemize}
    \item No-unets 
    \item \cite{Yi_2020} use an attention transfer module which is attention scores upsampled from $32 \times 32$.
    \item Supplement the U-net connection with a task-specific module \cite{Yan2018ShiftNet,Liu2020}
    \item \cite{Zhao2021} uses regular u-nets
    \item Shift-net \cite{Yan2018ShiftNet} a shift-module at the 32x32 resolution.
    \item AOT \cite{Zeng2022AOT} has a similar module, except for residual blocks.
\end{itemize}



==> tex/transformers.tex <==
\section{Inpainting with transformers.}

\textbf{Questions.}
\begin{itemize}
    \item Does it make sense for densely-guided inpainting? \eg the CSE embedding can help the encoder to "describe the image".
\end{itemize}

\textbf{The idea:} Following MAE \cite{He2022MAE}, compute budget of transformer-based models is signficantly reduced by removing patches that are masked out in the encoder.

\begin{figure}[h]
    \centering
    \includegraphics[width=.63\textwidth]{figures/transfomer_mask_size.pdf}%%
    \includegraphics[width=.37\textwidth]{figures/transfomer_mask_visualization.png}
    \caption{
        Histogram of the percentage of visible pixels in the image for the FDH validation dataset.
        \textbf{Right:} Original mask, the enlarged mask and the shrunk mask.
    }
\end{figure}

\begin{figure}[h]
    \includegraphics[width=\textwidth]{figures/transfomer_mask_remaining_pixels.pdf}
\end{figure}
Training transformers, we need a fixed length input. MAE uses ~75\% masking ratio, \ie only 25\% of the image is inputted to the encoder.

Design decisions:
\begin{itemize}
    \item A masking ratio.
    \item A transformer can infer a "draft of the scene", but will generate poor results where we have removed masks.
    \item We can train the transformer with more masks than required, but can reduce it during inference?
\end{itemize}



